Joint Learning of Hierarchical Community Structure and Node Representations: An Unsupervised Approach

Graph representation learning has demonstrated improved performance in tasks such as link prediction and node classification across a range of domains. Research has shown that many natural graphs can be organized in hierarchical communities, leading to approaches that use these communities to improve the quality of node representations. However, these approaches do not take advantage of the learned representations to also improve the quality of the discovered communities and establish an iterative and joint optimization of representation learning and community discovery. In this work, we present Mazi, an algorithm that jointly learns the hierarchical community structure and the node representations of the graph in an unsupervised fashion. To account for the structure in the node representations, Mazi generates node representations at each level of the hierarchy, and utilizes them to influence the node representations of the original graph. Further, the communities at each level are discovered by simultaneously maximizing the modularity metric and minimizing the distance between the representations of a node and its community. Using multi-label node classification and link prediction tasks, we evaluate our method on a variety of synthetic and real-world graphs and demonstrate that Mazi outperforms other hierarchical and non-hierarchical methods.

==> preamble.tex <==
\usepackage[utf8]{inputenc}


\usepackage[usenames, dvipsnames]{color}
\usepackage{amsmath}
\usepackage{booktabs}
\usepackage{array}
\setlength\extrarowheight{2pt}
\usepackage{bbm}
\usepackage{algorithmic}

%\usepackage[]{color-edits}
% \usepackage[suppress]{color-edits}
%\addauthor{ast}{green}

%-----------------------------------------------------------
% PACKAGES AND COMMANDS NEEDED FOR TABLES
%-----------------------------------------------------------
\usepackage{tabularx} % nice format for tables, has X command for auto spacing between columns


==> sec-framework-copy.tex <==
\section{\mazi Framework}
\label{sec:proposed-copy}

%\subsection{Overview}

The \emph{Mazi} framework seeks to jointly learn the node representations and the community structure of the graph at each level in the hierarchy. 
%
To do so, the objective function in \emph{Mazi} is formulated using three major components. First, for each node, captured within its representation, the proximity to its neighborhood is modeled using a Skip-gram objective. Next, a second component is added to maximize the proximity of the node to its direct lineage in the embedding space. Finally, a third component is added that models and learns the hierarchical community structure of the graph.

The graph $G$ is progressively coarsened as an initialization to the hierarchical community structure. 
%To achieve this, we generate its communities at each level using existing community detection algorithms and collapse the graph to form coarser graphs at that level. 
Alongside, representations for the coarsened nodes are computed for all the levels in the hierarchy. Then, using an alternating optimization approach in a level-by-level fashion, the objective at each level is optimized using the above. First, the community structure at a level is held fixed and used to influence the node representation, and then, the node representations, held fixed, is used to refine the community structure of the graph at that level.
%
The optimization updates step through the levels in the hierarchy from the finest graph to the coarsest graph, referred to as \emph{Forward Optimization}, and then from the coarsest graph to the finest graph, referred to as \emph{Backward Optimization}, enabling the node representations at each level to align itself to its direct lineage in the embedding space, additionally refining the community structure by the information contained within this embedding space. An illustration of the framework is shown in Figure~\ref{fig:mazi_fd}. 

\begin{figure*}
  \includegraphics[width=\textwidth]{images/hier_lvl_vertical_1102.pdf}
  \caption{The different steps in \emph{Mazi} are illustrated. The original graph at level $1$ is coarsened twice resulting in $3$ overall levels. At each level, \emph{Mazi} alternatively optimizes the representations, $X$, and the clustering solution, $H$, in a level-by-level fashion. %Specifically, \emph{Mazi} first learns the representations for the nodes in that level, $l$, $X^{l}$, and then recomputes the clustering solution for that level, $H^{l}$. 
  Specifically, at level $1$, \emph{Mazi} updates $X^1$ followed by $H^1$, then moves in the forward direction to level $2$, to update $X^2$ and $H^2$. This is then followed by optimization steps in the backward direction, that is, first at level $2$ and then level $1$.
  Level $3$ can be viewed as an all encompassing node, whose representation, $X^3$, is an average of the representations of all the nodes in the original graph, and serves as a reference point to align node representations at finer levels. 
  %This node is used a location in the embedding space around which we expect the hierarchical representations to align.
  Initializations for the representations and the clustering solution at level $l$ is denoted by $X^l$ and $H^l$. 
  Updated node representations at level $l$ is denoted by $X^{l}'$ and updated clustering solution at level $l$ is denoted by $H^{l}'$. 
  }
  \label{fig:mazi_fd}
\end{figure*}

\iffalse
 By performing the optimization in the backward direction such as above, we ensure that the representations of nodes in the finer levels of the hierarchy are influenced by the representations of the nodes in the coarser levels of the hierarchy. Moreover, in each sub-problem $H^l$, by jointly optimizing the \emph{modularity} objective with that of minimizing the distance between the node representation and its community representation, we ensure that the communities in each level are informed by the representations of the nodes involved as well. The outline of our overall algorithm can be found in Algorithm~\ref{mazi}.
\fi

%Further, we utilize a highly efficient approach to refine the community structure. The rest of the section will  proceed to explain the three components discussed above and our algorithm in more detail. 
%which we minimize utilizing alternating optimization in a level-by-level fashion. 
%The rest of the section will introduce the notations and the prelimiaries required for the model and then proceed to explain the three components discussed above. 

%\input{sec-prelim}

\begin{comment}
In this section, we present our algorithm, \emph{Mazi} we designed to jointly learn the node embeddings and the hierarchical community structure of the graph. We formulate our objective utilizing three components. First, we use the Skip-gram model to model the node neighborhood. To this, we add a second component that maximizes the node proximity to its direct lineage. The third component that we add to the objective aids to model and learn the hierarchical community structure of the graph. 
%which we minimize utilizing alternating optimization in a level-by-level fashion. 

Our algorithm reads an undirected graph in the edgelist format and extracts the largest connected component from the same. We create an induced sub-graph using the nodes that belong to the largest connected component by keeping the edges that connect the vertices in this component and discarding the rest and then, use this sub-graph for the rest of our algorithm. 
\textcolor{red}{We create an initial hierarchical community structure using this sub-graph and this pre-processing step ensures that the graphs constructed in the coarser levels further down in the hierarchy will remain connected.}
\end{comment}

\subsection{Modeling Proximity to Neighborhood}
As previously studied, see~\cite{grover2016node2vec}, to capture the neighbourhood of a node in the representations, we seek to maximize the log-likelihood of observing the neighbors of a node conditioned on the representation of the node using the Skip-gram model with negative sampling.
%while minimizing the likelihood of encountering vertices that not in the neighborhood of that vertex. 

Utilizing the concept of sequence-based representations, neighboring nodes of a node $v$ are sampled to form its context. A weighted random-walk procedure is performed for each node a fixed number of times, denoted by $r$, wherein, the length of each of these walks is $l$ and $k$-sized contexts are extracted from these walks. Let the nodes contained in these contexts be represented by $N(v_i)$ for a node $v_i$. 

\iffalse
Furthermore, as in previous approaches, we assume two properties for learning these embeddings. First, for each node, encountering different neighboring nodes are independent conditioned on the representation of that node. Second, we assume symmetry in the embedding space. 
\fi
%
Further, let the representation of a node $v_i$ be denoted by $x_i$ and its neighbor, $v_j$ such that $v_j \in N(v_i)$, be denoted by $x_j$. 
The negative sampling distribution of the vertex $v_i$ is denoted by $P_n$ and the number of negative samples considered for training the loss is denoted by $R$. 
\iffalse
\begin{equation}
%\begin{gather*}
\begin{split}
\label{negsamp}
\max_{x_i}~L_{nbr} = \frac{1}{|N(v_i)|}\big(\sum_{v_j\in{N(v_i)}}\log \sigma(x_i \cdot x_j) \\
        +~R \cdot E_{v_n \sim  P_n(v_i)}-\log \sigma(x_i \cdot x_j)\big)
\max_{x_i}~L_{nbr} = \big(L_{nbr\_pos}+L_{nbr\_neg}\big)
\end{split}
%\end{gather*}
\end{equation}
\fi
%
We use $L_{nbr\_pos}$ to denote the loss of $v_i$ to its neighbors and $L_{nbr\_neg}$ to denote the loss of $v_i$ to its negative samples. Using the above, we define $L_{nbr\_pos}$ and $L_{nbr\_neg}$ as,
\begin{subequations}
%\begin{gather*}
%\begin{split}
\begin{align}
\label{negsamp}
L_{nbr\_pos} &= \frac{1}{|N(v_i)|}\sum_{v_j\in{N(v_i)}}\log \sigma(x_i \cdot x_j) \label{pos_loss}\\
L_{nbr\_neg} &= ~R \cdot E_{v_n \sim P_n(v_i)}\log (1-\sigma(x_i \cdot x_j)) \label{neg_loss}
\end{align}
%\end{split}
%\end{gather*}
\end{subequations}

Taken together, we model the neighbourhood proximity of a node $v_i$ as, 
\begin{equation}
\begin{split}
\max_{x_i}~L_{nbr} &= L_{nbr\_pos}~+~L_{nbr\_neg} 
\end{split}
\end{equation}



\iffalse
Furthermore, as in previous approaches, we also assume two properties for learning these embeddings. 
Let the representation of a node $v_i$ be denoted by $x_i$ and its neighbor, 
$v_j$ such that $v_j \in N(v_i)$, be denoted by $x_j$. 
First, we assume that for each node, encountering different neighboring nodes are 
independent conditioned on the representation of that node.  
This allows us to factorize the likelihood of a vertex $v_i$ as follows, 

\begin{equation}
\label{cond_ind}
P(N(v_i)|x_i) = \prod_{v_j\in{N(v_i)}} P(v_j|x_i, x_j)
\end{equation}
\noindent
Second, our model also assumes the symmetry in the embedding space. Using a softmax function, Equation~(\ref{cond_ind}) can be expressed as below, 
\begin{equation}
\label{ovli}
 P(v_j \in N(v_i)|x_i, x_j) = \frac{\exp(x_i \cdot x_j)}{\sum_{v_k \in V}\exp(x_i \cdot x_k)}
\end{equation}
\noindent
Since the denominator is computationally expensive, we use negative sampling in the objective. Replacing log likelihood to model the neighbourhood preserving objective, for a node  $v_i$ we get, 
\vspace{-3em}
\begin{equation}
    \label{negsamp}
    \max_{x_i}\frac{1}{|N(v_i)|}\big(\hspace{-2mm}\sum_{v_j\in{N(v_i)}}\hspace*{-3mm}\exp(x_i \cdot x_j) + 
        ~R \cdot E_{v_n \sim  P_n(v_i)}-\exp(x_i \cdot x_n)\big)
\end{equation}

%Such vertices whose distances are maximized are referred to as negative samples. 
 %$N(v_i^l)$ denotes the set of vertices that form the neighborhood of $v_i^l$, 
 \noindent
 Here, $P_n$ in the Sub-equation~(\ref{negsamp}) represents the negative sampling distribution of the vertex $v_i$, and $R$ describes how many negative samples will be considered for training the loss. Moreover,
 \begin{equation} \label{eq:s}
 \sigma(x) = \frac{1}{1 + e^{-x}}
 \end{equation} 
 is the sigmoid function.
 %Note that \begin{equation} \label{eq:s}
 %\sigma(x) = \frac{1}{1 + e^{-x}}
 %\end{equation} 
 %is the sigmoid function.
 \fi
 %
 
 \subsection{Modeling Proximity to Community}
 
 %Let the total number of levels in the hierarchical community structure of the graph be $L$. \textcolor{red}{$L$ is a parameter that is tuned in our algorithm.} Consider one of those levels, $l$, in our hierarchical representation. 
 %Let the representation of a node $v_i^l$ in level $l$ be denoted by $x_i^l$, its neighbors by $v_j^l$ and  their corresponding representations by $x_j^l$. 
 %
 %We utilize the term~(\ref{eq:1term2}) in the formula to denote the relationship between the vertex representation $x_i^l$ and its associated community, whose representation is denoted by $x_{H^l(v^l_i)}^{l+1}$. 
 %
 Nodes belonging to a community is similar to each other in comparison with nodes lying outside the community. As a consequence, we expect the representation of a node to be similar to the representation of its lineage in the hierarchical structure, that is, its associated community in the subsequent level and to its children in the previous level. 
 %
 %Let the total number of levels in the hierarchical community structure of the graph be $L$. 
 Consider a level, $l$, in the hierarchical community structure of a graph. Let the representation of a node $v_i^l$ in level $l$ be denoted by $x_i^l$. Further, let the representation of its associated community in the next level $l+1$ be denoted by $x_{H^l(v^l_i)}^{l+1}$. Here, $H^l(
 v^l_i)$ is the community membership indicator of the node $v^l_i$ in the level $l$ in the hierarchy.
 It is a vector of size $|V^l|$ and takes a discrete value between $[0 \dots k^l-1]$, where $k^l$ is the number of communities in level $l$, or, the number of nodes in level $l+1$.
 %$l+1$ and the modular structure present 
 %in that level in the embedding space is captured.
 %
 To model the relationship between the node $v^l_i$ and its associated community $H^l(v^l_i)$, we use,
 \vspace{-3mm}
 \begin{equation}
 \label{comm_level}
    \max_{x^l_i}~L_{comm}~=~\log \sigma\big(x_i^l \cdot {x_{H^l(v_i^l)}^{l+1}}\big)
 \end{equation}
 
 As we progress up the hierarchy of the graph, with each passing level, we bring together nodes in each level closer to its parent node in the subsequent level in the embedding space. Resultingly, the representation of a node is influenced by the different communities the node belongs to at multiple resolutions. 
 %is a matrix of size $|V^l| \times k^l$, where $k^l$ is the number of communities in level $l$.
 
 %In order to also apply such an objective to the vertices in the level $L$, we set $x_{H^l(v^l_i)}^{L+1}$ as a vector of all-ones. This corresponds to the coarsest graph representation, and can be viewed as the representation of an all-encompassing community with all the vertices contained inside it. Therefore, we learn the representations of the vertices in different levels around this all-ones vector. 
 
\subsection{Jointly Learning the Hierarchical Community Structure and Node Representations}

 %In the above sections, we detail how we utilize a static community structure to inform and improve the node representations. Now, communities in a graph are typically generated by utilizing the topological structure of the graph. 
 Typically, community detection algorithms utilize the topological structure of the graph to generate clustering solutions. In addition to the topology of the graph, however, we may also take advantage of the information contained within the representations learned for each node to better the communities generated. 
 %
 At each level in the hierarchy, with the representations learnt, we refine and improve the community structure by leveraging the representations of the nodes as well. With such a refinement, the communities that we learn at each level in the hierarchy of a graph better align with the structural and the functional components of the graph at that level.   
  
 %By doing this, we get the benefit of ensuring that the communities formed in that level
 %are influenced\textcolor{red}{(/informed)} by the node representations learned.
 
 To refine the communities present in level $l$ using the representations of the nodes for that level, we add the \emph{modularity} objective, described previously, to the overall objective. At each level, we use, 
 \begin{equation}
 \label{mod_level}
 Q^l = ~\frac{1}{d(V^l)}\Big(\sum_{H^l_i \in H^l}(d_{int}(H^l_i) - \frac{d(H^l_i)^2}{d(V^l)})\Big)\Bigg)     
 \end{equation}
 
 
 %the node representations capture the modular structure present 
 %in the graph while preserving the global structure. 
 %
\iffalse
 \input{forward_backward_objective}
\fi

\iffalse
 % Squeezed.
 \begin{subequations}
 \label{eqn_dbl_x}
    \begin{align}
        \hspace*{-6mm}{\max_\theta} \sum_{l=1}^{L}\hspace*{-1mm}\Bigg(\frac{1}{|V^l|}\hspace*{-1mm}\sum_{v_i^l\in{V^l}}\hspace*{-1mm}\Big(\frac{1}{|N(v_i^l)|}\hspace*{-1mm}\sum_{v_j^l\in{N(v_i^l)}}\hspace*{-3mm}\log \sigma(x_i^l \cdot x_j^l)~+ \label{eq:1term1a}  \\
        \hspace*{-3cm}\alpha^l~R^l \cdot E_{v_n^l \sim  P_n^l(v_j^l)}(\log \sigma(-x_i^l \cdot x_n^l))~+ \label{eq:1term1b} \\
        \beta^l~(\log \sigma(x_i^l \cdot {x_{H^l(v_i^l)}^{l+1}}) \Big)~+  \label{eq:1term2} \\
        \gamma^l~\frac{1}{d(V^l)}\Big(\sum_{H^l_i \in H^l}(d_{int}(H^l_i) - \frac{d(H^l_i)^2}{d(V^l)})\Big)\Bigg), \label{eq:1term3} \\
        %x^{L+1}_{H^l(v_i^l)} = \vec{1},\\
        ~\theta = x_i^l, H^l, \\
        i \in 1 \dots |V|^l~~\forall l \in 1 \dots L
    \end{align}
 \end{subequations}
 \fi
 
Consequently, putting all the components together and accounting for all the levels in the graph, we get the following coupled objective function,
\begin{equation}
\label{eqn_dbl_x}
    \begin{split}
       {\max_\theta} 
       ~\sum_{l=1}^{L} \Bigg(~&\frac{1}{|V^l|}\Big(L_{nbr\_pos} +\alpha^lL_{nbr\_neg}+\beta^lL_{comm}\Big)+\gamma^lQ^l\Bigg), \\
       &~\theta = x_i^l, H^l,~i \in 1 \dots |V|^l~~\forall l \in 1 \dots L
    \end{split}
    %\end{align}
\end{equation}

\iffalse
 \begin{subequations}
 \label{eqn_dbl_x}
    \begin{align}
        {\max_\theta} ~\sum_{l=1}^{L}\Bigg(~&\frac{1}{|V^l|}\sum_{v_i^l\in{V^l}}\Big(\frac{1}{|N(v_i^l)|}\sum_{v_j^l\in{N(v_i^l)}}\log \sigma(x_i^l \cdot x_j^l)~ \label{eq:1term1a}  \\
        & +~\alpha^l~R^l \cdot E_{v_n^l \sim  P_n^l(v_j^l)}(\log \sigma(-x_i^l \cdot x_n^l))~\label{eq:1term1b} \\
        & +~\beta^l~(\log \sigma(x_i^l \cdot {x_{H^l(v_i^l)}^{l+1}}) \Big)~  \label{eq:1term2} \\
        & +~\gamma^l~\frac{1}{d(V^l)}\Big(\sum_{H^l_i \in H^l}(d_{int}(H^l_i) - \frac{d(H^l_i)^2}{d(V^l)})\Big)\Bigg), \label{eq:1term3} \\
        %x^{L+1}_{H^l(v_i^l)} = \vec{1},\\
        &~\theta = x_i^l, H^l, \\
        &~i \in 1 \dots |V|^l~~\forall l \in 1 \dots L
    \end{align}
 \end{subequations}
\fi
\noindent
 
 %Note that the regularization parameters for the terms~(\ref{eq:1term1b}),~(\ref{eq:1term2}) 
 %Note that the various terms in the overall objective are normalized to be invariant to the input size and 
 Since the order of the three terms that contribute to the overall objective is different, the terms are normalized with its respective order of contribution. For instance, since the proximity of a node $v_i^l$ to its neighboring nodes is maximized in the Sub-equation~(\ref{pos_loss}), the contribution from this term will be dependent on the context size of that node. In comparison, when the proximity of the node to its associated community representation in the next level is maximized, captured by the Sub-equation~(\ref{comm_level}), the contribution of that single measure will be minor as compared to the summation over the measures that the Sub-equation~(\ref{pos_loss}) results in. This is especially true for larger values of context size. In similar light, $R^l$ needs to be scaled in order to ensure it does not dominate over other terms of the objective as well. 
 Further, $\alpha^l$, $\beta^l$ and $\gamma^l$ serve as regularization parameters and are added to the Sub-equations~(\ref{neg_loss}),~(\ref{comm_level}) and~(\ref{mod_level}) in the overall objective for each level $l$, respectively. 
 This is done so that the sub-equations are weighted with the
 optimal value of hyper-parameters which ensure that 
 different components in the objective contribute 
 equally to the overall value.       
 In summary, in our optimization problem, the parameters optimized includes the representations of vertices that belong to all the different levels ranging from $1\dots L$ and also the community membership for each of the vertices associated with these levels.
 %thereby, jointly learning the hierarchical community structure in the graph. 
 Therefore, this entire set of parameters, represented by $\theta$, is optimized in our objective function.
 
 \subsection{Algorithm}
 %In this section, we detail the efficient implementation of our algorithm.
 \subsubsection{Optimization Strategy}
 We utilize an alternating optimization (AO) approach to optimize our formulation. We perform AO in a level-by-level fashion, by fixing variables belonging to all the levels except one, say denoted by $l$, and optimizing the variables associated with that level. One set of variables at level $l$ include the community membership indicator vector, denoted by $H^l$, and the next set include the node representations, denoted by $X^l$. 
 %
 Thus, within a level $l$, we fix the community membership, $H^l$, and update the node representations $X^l$. Then, we fix $X^l$, and update $H^l$. 
 
 \subsubsection{Node Representation and Community Structure Initializations}
 Let us denote the node representation update as the $X^l$ sub-problem, and the community membership update as the $H^l$ sub-problem. 
 %We start with an initial solution for each of the above sub-problems and use our algorithm to further optimize them. %
 %
 \iffalse
 We initialize the node representations at the finest level of the graph, denoted by parameters $X^1$, by learning representations from an embedding method such as \emph{node2vec}~\cite{grover2016node2vec}. Further, we generate an initial community membership for the finest level, denoted by $H^1$, by using existing community detection algorithms such as \emph{Nerstrand}~\cite{lasalle2013nerstrand} or \emph{Metis}~\cite{karypis1995multilevel}. 
 \fi
 %
  The node representations at the finest level of the graph, denoted by $X^1$, are initialized by learning representations from an embedding method such as \emph{node2vec}~\cite{grover2016node2vec}. Further, an initial community membership for the finest level, denoted by $H^1$, is generated by using existing community detection algorithms such as \emph{Nerstrand}~\cite{lasalle2013nerstrand} or \emph{Metis}~\cite{karypis1995multilevel}. 
 %
 %
 With these initializations, 
 %of representations, $X^1$, and the community membership, $H^1$, 
 the node representations, $X^l$, and community structure, 
 $H^l$, for each level $l$ in the hierarchy is generated. 
 The graph is coarsened at each subsequent level, $l$, by creating super-nodes, denoted by $v^l_i$, by collapsing all the nodes that are assigned to $v^l_i$ at level $l-1$, that is, $H(v_j^{l-1})=v^l_i$.
 %
 %using the community structure from the previous level such that the current level merges nodes assigned to the same community from the previous level to form super nodes.
 Further, for the resulting coarse graph at level $l$, the edges are formed by collapsing all the edges from the previous level, $l-1$, such that it forms an edge between the super-nodes (communities) in this level, $l$.  The edge weights at level $l$ corresponds to the number of edges that have been collapsed to an edge between a pair of super-nodes in this level. Line 3-8 in Algorithm~\ref{init_ghx} corresponds to these steps.
 %First, at a level $l$, we create a super-node, $v^l_i$, by merging all the nodes that are assigned to $v^l$ at level $l-1$, that is, $H(v^{l-1})=v^l_i$. 
 %
 Next, consider a node in level $l$, denoted by $v^l$. The representation for $v^l$ is computed by the taking the average of the representations of the nodes in level $l-1$ that are assigned to the community(super node) $v^l$ in the level $l$. In Algorithm~\ref{init_ghx}, Line 9-10 corresponds to these steps. Finally, in Line 12, we describe how for the resulting coarsened graph at level $l$, we run the chosen community detection algorithm again to form initialization of the community structure for the next level $l+1$. Our pseudocode to generate the initializations for the hierarchical community structure and the representations can be referred to in Algorithm~\ref{init_ghx}.
 
\iffalse
 We next discuss the update equations for the $X^l$ sub-problem. 
 \textcolor{red}{
 First, we find the derivative with respect to $x^l_i$. Let $NS$ be the set of negative samples drawn from the negative sample distribution denoted by $P(v^l_j)$. For each vertex $v^l_i$, we get the following: 
 \\\\
\begin{subequations}
\begin{align}
\frac{\partial X^l}{\partial x^l_i} = \sum_{v_j \in N(v_i)} (1 - \sigma(||x^l_i - x^l_j||_2)) \frac{x^l_i - x^l_j}{||x^l_i - x^l_j||_2} \\
 - Q~\frac{1}{|NS|}\sum_{v^l_n \sim P(v^l_j)}\sigma(||x^l_i - x^l_n||_2)\frac{x^l_i - x^l_n}{||x^l_i - x^l_n||_2} \\ 
 + \frac{x^l_i - x^{l+1}_{H^l(v^l_i)}}{||x^l_i - x^{l+1}_{H^l(v^l_i)}||_2}
\end{align}
\end{subequations} 
\noindent
Next, we find the derivatives with respect to $x^l_j$. Here, for a vertex $v^l_i$ and for one of its neighbor $v^l_j$, we get the following update equation: 
\\\\
\begin{subequations}
\begin{align}
\frac{\partial X^l}{\partial x^l_j} = -\sum_{v_j \in N(v_i)} (1 - \sigma(||x^l_i - x^l_j||_2)) \frac{x^l_i - x^l_j}{||x^l_i - x^l_j||_2} 
\end{align}
\end{subequations} 
\noindent 
Finally, we find the derivative with respect to $x^l_n$. For each vertex $v^l_i$, we get the following update: 
\\\\
\begin{subequations}
\begin{align}
\frac{\partial X^l}{\partial x^l_n} = Q~\frac{1}{|NS|}\sum_{v^l_n \sim P(v^l_j)}\sigma(||x^l_i - x^l_n||_2)\frac{x^l_i - x^l_n}{||x^l_i - x^l_n||_2}
\end{align}
\end{subequations} 
\\}
\fi
\subsubsection{Node Representation and Community Structure Refinement}
At each level $l$, we first find the gradient updates for the $X^l$ sub-problem in our model. In our implementation, we use the ADAM optimization algorithm~\cite{kingma2014adam} to update the weights. 
Then, we optimize the $H^l$ sub-problem while also using the updated $X^l$ in level $l$. Specifically, in our algorithm, we utilize an efficient move-based approach to maximize the \emph{modularity} objective while minimizing the distance of each vertex to its associated community to generate communities informed by their node representations. Although the computation of \emph{modularity} is expensive, utilize a fast algorithm that can scale to very large graphs which we describe next. Let the number of communities be denoted by $|H^l|$. Recall from the Subsection~\ref{sec:prelim} that the \emph{modularity}, $Q$, for a community membership solution $H$ is given by, 
\begin{equation}
 Q = \frac{1}{d(V)}\Bigg(\sum_{h_i \in H}\bigg(d_{int}(h_i) - \frac{d(h_i)^2}{d(V)}\bigg)\Bigg).
\end{equation}
Here, we note that $Q$ can be computed by computing the internal degree and external degree of all communities and applying the above equation. Therefore, to move $v^l_i$ from a community $h^l_i$ to another $h^l_j$, instead of computing the modularity contribution from each community, we observe that an efficient way to perform this is to only modify the internal and the external degree of communities $h^l_i$ and $h^l_j$ by computing how the contribution of $v^l_i$ to $h^l_i$ and $h^l_j$ change, respectively. 
%To move a node $v^l_i$ from its community $H^l(v^l_i)$ to another community such that it maximizes the overall \emph{modularity}, 
To this end, for each node $v^l_i$ in level $l$, we first compute the degree of $v^l_i$ independently to all the $|H^l|$ communities. Let us denote the degree $v^l_i$ forms with a community $h_j$ as $deg_{v^l_i}[h_j]$. 
Thus, the overall degree of the node is given by the following,  
\begin{equation}
    deg(v^l_i) = \sum_{j \in |H^l|} deg_{v^l_i}[h_j].
\end{equation} 
For a node, this step will be of cost $O(deg(v^l_i))$.
We then loop over all communities $h^l_i \in H^l$ such that $h^l_i \neq H^l(v^l_i)$ and evaluate if the node $v^l_i$ should be moved to  to community $h^l_i$ to maximize the \emph{modularity}. 
Since we are removing $v^l_i$ from community $H^l(v^l_i)$, we modify the external degree of $H^l(v^l_i)$ by removing the entire degree contribution of $v^l_i$ and adding twice the internal degree contribution of $v^l_i$ to the same. In similar light, to move $v^l_i$ to $h^l_i$, we remove twice the degree contribution of $v^l_i$ to $h^l_i$ from the external degree of $h^l_i$, and add the entire degree contribution of $v^l_i$. The internal degree of the two communities is easier to modify, that is, we remove the internal degree  contribution of $v^l_i$ from $H^l(v^l_i)$ and add the same to community $h^l_i$. This entire set of operations is of the order $O(k)$, since the cost of looking up the node degree contributions and modifications of the internal and the external degree contribution is $O(1)$.
%Then, for each community $h^l_i$, such that $h^l_i \neq H^l(v^l_i)$,  we remove the degree contribution of $v^l_i$ from the internal and the external degree of $H^l(v^l_i)$ and add the contribution to the internal and external degree of community $h^l_i$. 
Using this efficient sequence of computations, we determine the new community assignment of node $v^l_i$ such that it maximizes $Q$. Note that along with $Q$, we also couple the minimization of distance of the node representation to that of its parent in the objective and choose the assignment that maximizes the overall objective. This step is also easy to compute since, for each vertex, we only need to modify the contribution of this distance to evaluate each community reassignment. Also note that the actual move will require updates of the internal and the external degree contribution of the node to the different communities. This step is also of the order $O(1)$. This entire process is repeated for all nodes multiple times until no moves lead to a better $Q$ value. We then return this as the optimized solution for the $H$ sub-problem. 

\iffalse
This implies that the degree of $v^l_i$, denoted by $deg(v^l_i)$, is  
\begin{equation}
    deg(v^l_i) = \sum_{j \in |H^l|} deg_{v^l_i}[h_j]
\end{equation}
\fi

\iffalse
Further, let the degree of a vertex $v^l_i$ be denoted by $deg(v^l_i)$, and the edge set in the graph at level $l$ be $E^l$. 
Specifically, we utilize a move-based approach to maximize the modularity objective coupled with minimizing the distance of each vertex to its associated community. \textcolor{red}{This is detailed in algorithm ..} where, $Q$ is the modularity objective which was previously described in Section~\ref{background}.
\fi

After having alternatively solved for the sub-problems $X$ and $H$ in level $l$, we optimize level $l+1$, and so on until we reach level the last level $L$. On reaching level $L$, we then optimize the node representations of the coarsest graph, not including the single-node coarse graph, in the backward direction level-by-level using the updated representations, that is, $L-1$, $L-2$, $\dots$, 1. By performing the optimization in the backward direction such as above, we ensure that the representations of nodes in the finer levels of the hierarchy are influenced by the representations of the nodes in the coarser levels of the hierarchy. Moreover, in each sub-problem $H^l$, by jointly optimizing the \emph{modularity} objective with that of minimizing the distance between the node representation and its community representation, we ensure that the communities in each level are informed by the representations of the nodes involved as well. The outline of our overall algorithm can be found in Algorithm~\ref{mazi}. 


\begin{algorithm}
\caption{InitializeGXH}
\begin{algorithmic}[1]
\label{init_ghx}
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE $G^1=(V^1, E^1, W^l)$ - the finest level graph,
 \\ \hspace{0.5cm}$X^1$ - the node representations at the finest level,
 \\ \hspace{0.5cm}$H^1$ - the clustering solution at the finest level, 
 \\ \hspace{0.5cm}$L$ - the number of levels.
 \ENSURE  $G^l=(V^l, E^l, W^l)$, $H^l$, $X^l$, for $l \in [1 \dots L]$
 \FOR{$l$ = $1$~\TO~$L-1$} 
    \FOR{$h$ = $1$~\TO~$|H^l|$}
        \STATE {Merge node $v^l$ to node $v^{l+1}_h$, \\ where $v^{l+1}_h$ represents $h$ in layer $l+1$, 
        \\ $v^l \in V^l$, $H^l[v^l] == h$}
        %\STATE {Coarsen graph for level $l$, $G^l$, where, nodes are represented by $V^l$, and $|V^l| = |H^{l-1}|$ and edges $E^l$, are         represented by the inter-community edges of $H^{l-1}$.} \\
    \ENDFOR
    \FOR{$(v_i, v_j) \in E^l$}
        \STATE {Add $(v^{l+1}_{H(v_i)}, v^{l+1}_{H(v_j)})$ to $E^{l+1}$}
        \STATE {$w^{l+1}_{(v^{l+1}_{H(v_i)}, v^{l+1}_{H(v_j)})} += w^{l}_{(v_i^{l}, v_j^{l})}$}
    \ENDFOR
    \FOR{$v_i^l \in V^l$}
        \STATE{$x^{l+1}_{v^{l+1}_{H(v_i)}} += x^l_{v^l_i}$}
    \ENDFOR
    \STATE{Generate $H^{l+1}$ for $G^{l+1}(V^{l+1}, E^{l+1}, W^{l+1})$.}
\ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{UpdateXH}
\begin{algorithmic}[1]
\label{update_hx}
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE $G^l=(V^l, E^l, W^l)$ - the graph at level $l$,\\ 
 \hspace{0.5cm}$X^{l-1}, X^l, X^{l+1}$ - the node representations at \\ 
 \hspace{1.5cm}level $l-1$, $l$, $l+1$, \\ 
 \hspace{0.5cm}$H^{l-1}, H^l, H^{l+1}$ - the clustering solution at \\
 \hspace{1.5cm}level $l-1$, $l$, $l+1$, \\ 
 \hspace{0.5cm}$k$ - the context size to extract from the walks, \\ 
 \hspace{0.5cm}$l$ - the length of random-walk, \\
 \hspace{0.5cm}$r$ - number of walks per node, \\
 \hspace{0.5cm}$L$ - number of layers in the hierarchy, \\
  \hspace{0.5cm}$lr$ - learning rate at level $l$, \\
 \hspace{0.5cm}$n$ - number of epochs at level $l$, \\
 \hspace{0.5cm}$d$ - embedding dimension, \\
 \hspace{0.5cm}$\alpha$ - contribution of node neighborhood to overall loss, \\
 \hspace{0.5cm}$\beta$ - contribution of proximity to parents to overall loss, \\
 \hspace{0.5cm}$\gamma$ - contribution of modularity to overall loss. \\
 \ENSURE  $X^l$, $H^l$
 \FOR{$v_i \in V^l$}
  \FOR{$walk\_num = 1$~\TO~$r$}
    \STATE {$train\_sequences$ \gets RandomWalker$(G^l, k, l)$}
    \STATE {$X^l$ \gets UpdateX($X^{l-1}, H^{l-1},$ $X^{l}, H^{l}, X^{l+1}, H^{l+1},$ \\ \hspace{1.00cm}$train\_sequences, n, lr, \alpha,$ $\beta)$}
  \ENDFOR
 \ENDFOR
 \STATE {$H^l \gets UpdateH(G^l, X^{l}, H^{l}, X^{l+1}, H^{l+1}, \beta, \gamma)$}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{MoveTo}
\begin{algorithmic}[1]
\label{moveto}
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE $v_i$ - the vertex to be moved,
 \\ \hspace{0.5cm}$h_{to}$ - the destination community,
 \\ \hspace{0.5cm}$h_{from}$ - the source community, 
 \\ \hspace{0.5cm}$degrees$ - the degree of $v_i$ to all communities,
 \\ \hspace{0.5cm}$ID$ - internal degree of all communities,
 \\ \hspace{0.5cm}$ED$ - external degree of all communities,
 \\ \hspace{0.5cm}$deg(v_i)$ - degree of node $v_i$.
 \ENSURE  $objective$
 \STATE{$ED[h_{from}]$ = $ED[h_{from}]-deg(v_i) +  degrees[h_{from}]$}
 \STATE{$ED[h_{to}]$ = $ED[h_{to}]-degrees[h_{to}] + deg(v_i)$}
 \STATE{$ID[h_{from}]$ = $ID[h_{from}]-degrees[h_{from}]$}
 \STATE{$ID[h_{to}]$ = $ID[h_{to}]+degrees[h_{to}]$}
 \STATE{$objective$ = ComputeQ($ID$, $ED$) - distance($x^l_{v_i}, x^{l+1}_{H({v_i})}$)}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{UpdateH}
\begin{algorithmic}[1]
\label{init_ghx}
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE $G=(V, E)$ - the finest level graph,
 \\ \hspace{0.5cm}$K$ - number of communities in the graph,
 \\ \hspace{0.5cm}$H$ - the current clustering solution of the graph,
  \\ \hspace{0.5cm}$X^{l}$ - the node representations of the graph at level $l$,
 \\ \hspace{0.5cm}$X^{l+1}$ - the node representations of the graph at level $l+1$.
 \ENSURE  $H$
    \FOR{$v_i \in V$}
        \STATE{Compute $degrees[k], k=1, \ldots (K)$}
        \STATE{$deg(v_i)$ = i32sum($degrees$)}
        \FOR{$k$ = $1$~\TO~$K$} 
            \STATE{$objectives[k]$ = MoveTo($v_i$, $k$, $H(v_i)$, $degrees$, ID, ED, $deg(v_i)$, $X$)}
            \STATE{$h_{max}$ = argmax($objectives$)}
            \STATE{Move $v_i$ to $h_{max}$ and update $ID$ and $ED$.}
        \ENDFOR
    \ENDFOR
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{The Mazi Framework}
\begin{algorithmic}[1]
\label{mazi}
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE $G^1=(V^1, E^1, W^1)$ - the original graph structure,\\ 
 \hspace{0.5cm}$X^1$ - the node representations for finest level, \\ 
 \hspace{0.5cm}$H^1$ - the clustering solution in the finest level, \\ 
 \hspace{0.5cm}$k$ - the context size to extract from the walks, \\ 
 \hspace{0.5cm}$l$ - the length of random-walk, \\
 \hspace{0.5cm}$r$ - number of walks per node, \\
 \hspace{0.5cm}$L$ - number of layers in the hierarchy, \\
 \hspace{0.5cm}$lr^1 \dots lr^L$ - learning rate per layer, \\
 \hspace{0.5cm}$n^1 \dots n^L$ - number of epochs per layer, \\
 \hspace{0.5cm}$W$ - iters in the forward and backward direction, \\
 \hspace{0.5cm}$d$ - embedding dimension, \\
 \hspace{0.5cm}$\alpha$ - contribution of node neighborhood to overall loss, \\
 \hspace{0.5cm}$\beta$ - contribution of proximity to parents to overall loss, \\
 \hspace{0.5cm}$\gamma$ - contribution of modularity to overall loss. \\
 \ENSURE  $X^l$, $H^l$, for $l \in [1 \dots L]$
 \STATE {$[G^1 \dots G^L], [X^1 \dots X^L], [H^1 \dots H^L]$ \gets InitializeGXH($G^1, X^l, H^1, L$)}
 \FOR{$w = 1$~\TO~$W$}
  \FOR{$l = 1$~\TO~$L-1$}
    \STATE{UpdateXH($G^l, X^{l-1}, H^{l-1}, X^{l}, H^{l}, X^{l+1}, H^{l+1}, lr^l, n^l, $
    \\ $d, \alpha, \beta, \gamma$)}
  \ENDFOR
  \FOR{$l = L-1$~\TO~$1$}
    \STATE{UpdateXH($G^l, X^{l-1}, H^{l-1}, X^{l}, H^{l}, X^{l+1}, H^{l+1}, lr^l, n^l, $ 
    \\ $d, \alpha, \beta, \gamma$)} 
  \ENDFOR
 \ENDFOR
\end{algorithmic}
\end{algorithm}



\iffalse
\[
M = \frac{1}{4|E|^l}~\sum_{(v^l_i, v^l_j) \in E^l}~\Big(A^l_{v^l_i, v^l_j} - \frac{deg(v^l_i)deg(v^l_j)}{2|E|^l}\Big)h_{v^l_i}h_{v^l_j}.
\]
Here, $h_{v^l_i}$ is set to $1$ when $v^l_i$ belongs to the considered community $k$, and $-1$ otherwise.
\fi

 
%By performing forward and backward optimizations such as above, we update vertex representations such that it is influenced by the hierarchy in both directions while learning the most optimal hierarchical structure.



